MobileAppScrutinator: A Simple yet Efficient Dynamic Analysis Approach for Detecting Privacy Leaks across Mobile OSs

Smartphones, the devices we carry everywhere with us, are being heavily tracked and have undoubtedly become a major threat to our privacy. As "tracking the trackers" has become a necessity, various static and dynamic analysis tools have been developed in the past. However, today, we still lack suitable tools to detect, measure and compare the ongoing tracking across mobile OSs. To this end, we propose MobileAppScrutinator, based on a simple yet efficient dynamic analysis approach, that works on both Android and iOS (the two most popular OSs today). To demonstrate the current trend in tracking, we select 140 most representative Apps available on both Android and iOS AppStores and test them with MobileAppScrutinator. In fact, choosing the same set of apps on both Android and iOS also enables us to compare the ongoing tracking on these two OSs. Finally, we also discuss the effectiveness of privacy safeguards available on Android and iOS. We show that neither Android nor iOS privacy safeguards in their present state are completely satisfying.

==> tikzlibraryshadows.blur.code.tex <==
%%
%% This is file `tikzlibraryshadows.blur.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pgf-blur.dtx  (with options: `texfile')
%% Copyright 2012 Martin Giese, martingi@ifi.uio.no
%% 
%% This file is under the LaTeX Project Public License
%% See CTAN archives in directory macros/latex/base/lppl.txt.
%% 
%% DESCRIPTION:
%%   `pgf-blur' adds blurred/faded/fuzzy shadows to TikZ/PGF
%% 


\def\fileversion{1.01}
\def\filedate{2012/04/24}
\message{ v\fileversion, \filedate}
\usetikzlibrary{shadows}
\usetikzlibrary{calc}
\tikzset{
  /tikz/shadow blur radius/.store in=\pgfbs@radius,
  /tikz/shadow blur radius=.4ex,
  /tikz/shadow blur extra rounding/.store in=\pgfbs@extra@rounding,
  /tikz/shadow blur extra rounding=\pgfutil@empty,
  /tikz/shadow blur extra rounding/.default=\pgfbs@radius,
  /tikz/shadow blur steps/.store in=\pgfbs@steps,
  /tikz/shadow blur steps=4,
  /tikz/shadow opacity/.store in=\pgfbs@opacity,
  /tikz/shadow opacity=40,
  /tikz/blur shadow/.style={
    shadow scale=1,
    shadow xshift=.5ex,
    shadow yshift=-.5ex,
    preaction=render blur shadow,
    every shadow,
    #1,
  },
  /tikz/render blur shadow/.code={
    \pgfbs@savebb
    \pgfsyssoftpath@getcurrentpath{\pgfbs@input@path}%
    \pgfbs@compute@shadow@bbox
    \pgfbs@process@rounding{\pgfbs@input@path}{\pgfbs@fadepath}%
    \pgfbs@apply@canvas@transform
    \colorlet{pstb@shadow@color}{white!\pgfbs@opacity!black}%
    \pgfdeclarefading{shadowfading}{\pgfbs@paint@fading}%
    \pgfsetfillcolor{black}%
    \pgfsetfading{shadowfading}%
       {\pgftransformshift{\pgfpoint{\pgfbs@midx}{\pgfbs@midy}}}%
    \pgfbs@usebbox{fill}%
    \pgfbs@restorebb
  },
}
\def\pgfbs@savebb{%
  \edef\pgfbs@restorebb{%
    \global\pgf@picminx=\the\pgf@picminx\relax
    \global\pgf@picmaxx=\the\pgf@picmaxx\relax
    \global\pgf@picminy=\the\pgf@picminy\relax
    \global\pgf@picmaxy=\the\pgf@picmaxy\relax
  }%
}
\def\restorebb{}%
\def\pgfbs@process@rounding#1#2{
  \expandafter\ifx\pgfbs@extra@rounding\pgfutil@empty%
    \pgfprocessround{#1}{#2}%
  \else%
    \pgfmathsetmacro\pgfbs@exrd@val{\pgfbs@extra@rounding}%
    \pgfbs@roundpath{#1}{\pgfbs@exrd@val pt}%
    \pgfsyssoftpath@getcurrentpath{\pgfbs@extraroundedpath}%
    \pgfprocessround{\pgfbs@extraroundedpath}{#2}%
  \fi%
}
\def\pgfbs@roundpath#1#2{%
  {%
    \def\pgfbs@rp@skipround{%
      \let\pgfbs@rp@possibleround\pgfbs@rp@insertround}%
    \def\pgfbs@rp@insertround{\pgfsyssoftpath@specialround{#2}{#2}}%
    \let\pgfbs@rp@possibleround\pgfbs@rp@insertround%
    %
    \def\pgfsyssoftpath@movetotoken##1##2{%
      \pgfsyssoftpath@moveto{##1}{##2}}%
    \def\pgfsyssoftpath@linetotoken##1##2{%
      \pgfbs@rp@possibleround\pgfsyssoftpath@lineto{##1}{##2}}%
    \def\pgfsyssoftpath@rectcornertoken##1##2##3##4##5{%
      \pgf@xa=##1\relax%
      \advance\pgf@xa by##4%
      \pgf@ya=##2\relax%
      \advance\pgf@ya by##5%
      \pgfsyssoftpath@moveto{##1}{##2}%
      \pgfbs@rp@possibleround%
      \pgfsyssoftpath@lineto{\the\pgf@xa}{##2}%
      \pgfbs@rp@possibleround%
      \pgfsyssoftpath@lineto{\the\pgf@xa}{\the\pgf@ya}%
      \pgfbs@rp@possibleround%
      \pgfsyssoftpath@lineto{##1}{\the\pgf@ya}%
      \pgfbs@rp@possibleround%
      \pgfsyssoftpath@closepath}%
    \def\pgfsyssoftpath@curvetosupportatoken%
       ##1##2##3##4##5##6##7##8{%
      \pgfbs@rp@possibleround%
      \pgfsyssoftpath@curveto{##1}{##2}{##4}{##5}{##7}{##8}}%
    \def\pgfsyssoftpath@closepathtoken##1##2{%
      \pgfbs@rp@possibleround\pgfsyssoftpath@closepath}%
    \def\pgfsyssoftpath@specialroundtoken##1##2{%
      \pgfmathsetmacro\pgfbs@rp@ra{max(##1,#2)}%
      \pgfmathsetmacro\pgfbs@rp@rb{max(##2,#2)}%
      \pgfsyssoftpath@specialround%
          {\pgfbs@rp@ra pt}{\pgfbs@rp@rb pt}%
      \let\pgfbs@rp@possibleround\pgfbs@rp@skipround%
    }
    #1%
  }
}
\def\pgfbs@compute@shadow@bbox{%
  \edef\pgfbs@minx{\the\pgf@pathminx}%
  \edef\pgfbs@miny{\the\pgf@pathminy}%
  \edef\pgfbs@maxx{\the\pgf@pathmaxx}%
  \edef\pgfbs@maxy{\the\pgf@pathmaxy}%
  \pgfmathsetmacro\pgfbs@midx{0.5*(\pgfbs@minx + \pgfbs@maxx)}%
  \pgfmathsetmacro\pgfbs@midy{0.5*(\pgfbs@miny + \pgfbs@maxy)}%
  \pgfmathsetmacro\pgfbs@minx{\pgfbs@minx - \pgfbs@radius}%
  \pgfmathsetmacro\pgfbs@miny{\pgfbs@miny - \pgfbs@radius}%
  \pgfmathsetmacro\pgfbs@maxx{\pgfbs@maxx + \pgfbs@radius}%
  \pgfmathsetmacro\pgfbs@maxy{\pgfbs@maxy + \pgfbs@radius}%
  \pgfmathsetmacro\pgfbs@wd{\pgfbs@maxx - \pgfbs@minx}%
  \pgfmathsetmacro\pgfbs@ht{\pgfbs@maxy - \pgfbs@miny}%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \pgfsyssoftpath@rect{\pgfbs@minx pt}{\pgfbs@miny pt}%
                      {\pgfbs@wd pt}{\pgfbs@ht pt}%
  \pgfsyssoftpath@getcurrentpath{\pgfbs@shadow@bbox}%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
}

\def\pgfbs@set@fading@pic@bbox{
  \global\pgf@picminx=\pgfbs@minx pt\relax
  \global\pgf@picminy=\pgfbs@miny pt\relax
  \global\pgf@picmaxx=\pgfbs@maxx pt\relax
  \global\pgf@picmaxy=\pgfbs@maxy pt\relax
}
\def\pgfbs@usefadepath#1{%
  \pgfsyssoftpath@setcurrentpath{\pgfbs@fadepath}%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfusepath{#1}%
}
\def\pgfbs@usebbox#1{%
  \pgfsyssoftpath@setcurrentpath{\pgfbs@shadow@bbox}%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfusepath{#1}%
}
\def\pgfbs@apply@canvas@transform{
  \pgflowlevel{
    \pgftransformshift{\pgfpoint{\pgfbs@midx}{\pgfbs@midy}}
    \pgftransformscale{\pgfkeysvalueof{/tikz/shadow scale}}
    \pgftransformshift{\pgfpoint%
      {\pgfkeysvalueof{/tikz/shadow xshift}-\pgfbs@midx}
      {\pgfkeysvalueof{/tikz/shadow yshift}-\pgfbs@midy}
    }
  }
}
\def\pgfbs@paint@fading{
  \pgfpicture
    % fix bounding box.
    \pgfbs@set@fading@pic@bbox
    % compute increments for line width and opacity
    \pgfmathsetmacro\pgfbs@op@step{50/\pgfbs@steps}
    \pgfmathsetmacro\pgfbs@wth@step{4*\pgfbs@radius/(2*\pgfbs@steps-1)}
    % draw the outer part of the fading,
    % starting with lightest, outermost line
    \pgfsetroundjoin
    \pgfmathsetmacro\pgfbs@max@i{\pgfbs@steps-2}
    \pgfmathsetmacro\pgfbs@wth{2*\pgfbs@radius}
    \pgfmathsetmacro\pgfbs@op{100-0.5*\pgfbs@op@step}
    \foreach \pgfbs@i in {0,...,\pgfbs@max@i} {
      \pgfsetlinewidth{\pgfbs@wth pt}
      \pgfsetstrokecolor{black!\pgfbs@op!pstb@shadow@color}
      \pgfbs@usefadepath{stroke}
      \pgfmathsetmacro\pgfbs@wth{\pgfbs@wth-\pgfbs@wth@step}
      \global\let\pgfbs@wth=\pgfbs@wth
      \pgfmathsetmacro\pgfbs@op{\pgfbs@op-\pgfbs@op@step}
      \global\let\pgfbs@op=\pgfbs@op
    }
    % clip to inside of path
    \scope
    \pgfbs@usefadepath{clip}
    % fill inside with final darkest shadow color
    \pgfsetfillcolor{pstb@shadow@color}
    \pgfbs@usebbox{fill}
    % draw the inner part of the fading,
    % starting with the darkest, innermost line
    \pgfmathsetmacro\pgfbs@wth{2*\pgfbs@radius}
    \pgfmathsetmacro\pgfbs@op{0.5*\pgfbs@op@step}
    \foreach \pgfbs@i in {0,...,\pgfbs@max@i} {
      \pgfsetlinewidth{\pgfbs@wth pt}
      \pgfsetstrokecolor{black!\pgfbs@op!pstb@shadow@color}
      \pgfbs@usefadepath{stroke}
      \pgfmathsetmacro\pgfbs@wth{\pgfbs@wth-\pgfbs@wth@step}
      \global\let\pgfbs@wth=\pgfbs@wth
      \pgfmathsetmacro\pgfbs@op{\pgfbs@op+\pgfbs@op@step}
      \global\let\pgfbs@op=\pgfbs@op
    }
    \endscope
    % a final stroke to hide clip/antialiasing artifcats
    \pgfsetstrokecolor{black!50!pstb@shadow@color}
    \pgfsetlinewidth{0.5*\pgfbs@wth@step}
    \pgfbs@usefadepath{stroke}
  \endpgfpicture
}
\endinput
%%
%% End of file `tikzlibraryshadows.blur.code.tex'.

